FishEye8K: A Benchmark and Dataset for Fisheye Camera Object Detection

With the advance of AI, road object detection has been a prominent topic in computer vision, mostly using perspective cameras. Fisheye lens provides omnidirectional wide coverage for using fewer cameras to monitor road intersections, however with view distortions. To our knowledge, there is no existing open dataset prepared for traffic surveillance on fisheye cameras. This paper introduces an open FishEye8K benchmark dataset for road object detection tasks, which comprises 157K bounding boxes across five classes (Pedestrian, Bike, Car, Bus, and Truck). In addition, we present benchmark results of State-of-The-Art (SoTA) models, including variations of YOLOv5, YOLOR, YOLO7, and YOLOv8. The dataset comprises 8,000 images recorded in 22 videos using 18 fisheye cameras for traffic monitoring in Hsinchu, Taiwan, at resolutions of 1080$\times$1080 and 1280$\times$1280. The data annotation and validation process were arduous and time-consuming, due to the ultra-wide panoramic and hemispherical fisheye camera images with large distortion and numerous road participants, particularly people riding scooters. To avoid bias, frames from a particular camera were assigned to either the training or test sets, maintaining a ratio of about 70:30 for both the number of images and bounding boxes in each class. Experimental results show that YOLOv8 and YOLOR outperform on input sizes 640$\times$640 and 1280$\times$1280, respectively. The dataset will be available on GitHub with PASCAL VOC, MS COCO, and YOLO annotation formats. The FishEye8K benchmark will provide significant contributions to the fisheye video analytics and smart city applications.

==> cvpr2023-author_kit-v1_1-1/latex/egbib.tex <==


@article{Alpher03,
author = {A. Alpher and J.~P.~N. Fotheringham-Smythe},
title = {Frobnication revisited},
journal = {Journal of Foo},
volume = 13,
number = 1,
pages = {234--778},
year = 2003
}

@article{Alpher04,
author = {A. Alpher and J.~P.~N. Fotheringham-Smythe and G. Gamow},
title = {Can a machine frobnicate?},
journal = {Journal of Foo},
volume = 14,
number = 1,
pages = {234--778},
year = 2004
}

@article{MIT-Car,
  title={A trainable system for object detection},
  author={Papageorgiou, Constantine and Poggio, Tomaso},
  journal={International journal of computer vision},
  volume={38},
  number={1},
  pages={15--33},
  year={2000},
  publisher={Springer}
}


@inproceedings{KITTI-D,
  title={Are we ready for autonomous driving? the kitti vision benchmark suite},
  author={Geiger, Andreas and Lenz, Philip and Urtasun, Raquel},
  booktitle={CVPR},
  pages={3354--3361},
  year={2012},
  organization={IEEE}
}

@inproceedings{CARPK,
  title={Drone-based object counting by spatially regularized regional proposal network},
  author={Hsieh, Meng-Ru and Lin, Yen-Liang and Hsu, Winston H},
  booktitle={ICCV},
  pages={4145--4153},
  year={2017}
}

@inproceedings{DGX-1, 
    title={Web-based multi-user concurrent job scheduling system on the shared computing resource objects}, url={http://dx.doi.org/10.1109/IIT50501.2020.9299110}, 
    DOI={10.1109/iit50501.2020.9299110}, 
    booktitle={14th International Conference on Innovations in Information Technology (IIT)}, 
    publisher={IEEE}, 
    author={Habuza, Tetiana and Khalil, Khaled and Zaki, Nazar and Alnajjar, Fady and Gochoo, Munkhjargal}, 
    year={2020}, 
    month={Nov} 
}

@inproceedings{UAVDT,
  title={The unmanned aerial vehicle benchmark: Object detection and tracking},
  author={Du, Dawei and Qi, Yuankai and Yu, Hongyang and Yang, Yifan and Duan, Kaiwen and Li, Guorong and Zhang, Weigang and Huang, Qingming and Tian, Qi},
  booktitle={ECCV},
  pages={370--386},
  year={2018}
}

@article{UA-DETRAC,
  author    = {Longyin Wen and
               Dawei Du and
               Zhaowei Cai and
               Zhen Lei and
               Ming{-}Ching Chang and
               Honggang Qi and
               Jongwoo Lim and
               Ming{-}Hsuan Yang and
               Siwei Lyu},
  title     = {{DETRAC:} {A} New Benchmark and Protocol for Multi-Object Tracking},
  journal   = {CoRR},
  volume    = {abs/1511.04136},
  year      = {2015},
  url       = {http://arxiv.org/abs/1511.04136},
  eprinttype = {arXiv},
  eprint    = {1511.04136},
  timestamp = {Mon, 13 Aug 2018 16:49:08 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/WenDCLCQLYL15.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{BDD100K,
  title={End-to-end learning of driving models from large-scale video datasets},
  author={Xu, Huazhe and Gao, Yang and Yu, Fisher and Darrell, Trevor},
  booktitle={CVPR},
  pages={2174--2182},
  year={2017}
}

@inproceedings{woodscape,
  title={{WoodScape}: A multi-task, multi-camera fisheye dataset for autonomous driving},
  author={Yogamani, Senthil and Hughes, Ciar{\'a}n and Horgan, Jonathan and Sistu, Ganesh and Varley, Padraig and O'Dea, Derek and Uric{\'a}r, Michal and Milz, Stefan and Simon, Martin and Amende, Karl and others},
  booktitle={ICCV},
  pages={9308--9318},
  year={2019}
}

@inproceedings{Sewer-ML,
  title={Sewer-ML: A Multi-Label Sewer Defect Classification Dataset and Benchmark},
  author={Haurum, Joakim Bruslund and Moeslund, Thomas B},
  booktitle={CVPR},
  pages={13456--13467},
  year={2021}
}

@article{AAURainSnow,
  title={Rain removal in traffic surveillance: Does it matter?},
  author={Bahnsen, Chris H and Moeslund, Thomas B},
  journal={IEEE Transactions on Intelligent Transportation Systems},
  volume={20},
  number={8},
  pages={2802--2819},
  year={2018},
  publisher={IEEE}
}

@inproceedings{Detection_in_LLC,
  title={Object detection in images with low light condition},
  author={Kvyetnyy, Roman and Maslii, Roman and Harmash, Volodymyr and Bogach, Ilona and Kotyra, Andrzej and aklin and Zhanpeisova, Aizhan and Askarova, Nursanat},
  booktitle={Photonics Applications in Astronomy, Communications, Industry, and High Energy Physics Experiments 2017},
  volume={10445},
  pages={104450W},
  year={2017},
  organization={International Society for Optics and Photonics}
}

@inproceedings{yu2020bdd100k,
  title={Bdd100k: A diverse driving dataset for heterogeneous multitask learning},
  author={Yu, Fisher and Chen, Haofeng and Wang, Xin and Xian, Wenqi and Chen, Yingying and Liu, Fangchen and Madhavan, Vashisht and Darrell, Trevor},
  booktitle={CVPR},
  pages={2636--2645},
  year={2020}
}

@article{MIO-TCD,
  title={MIO-TCD: A new benchmark dataset for vehicle classification and localization},
  author={Luo, Zhiming and Branchaud-Charron, Frederic and Lemaire, Carl and Konrad, Janusz and Li, Shaozi and Mishra, Akshaya and Achkar, Andrew and Eichel, Justin and Jodoin, Pierre-Marc},
  journal={IEEE Transactions on Image Processing},
  volume={27},
  number={10},
  pages={5129--5141},
  year={2018},
  publisher={IEEE}
}

@inproceedings{AI-City,
  title={The 5th ai city challenge},
  author={Naphade, Milind and Wang, Shuo and Anastasiu, David C and Tang, Zheng and Chang, Ming-Ching and Yang, Xiaodong and Yao, Yue and Zheng, Liang and Chakraborty, Pranamesh and Lopez, Christian E and others},
  booktitle={CVPR},
  pages={4263--4273},
  year={2021}
}

@misc{NEXET,
    author= {{Itay Klein, Nexar Blog}},
    year  = {2017},
    title = {{NEXET} - The Largest and Most Diverse Road Dataset in the World},
    note  = {\footnotesize{\url{https://data.getnexar.com/blog/nexet-the-largest-and-most-diverse-road-dataset-in-the-world}}, 
             Last accessed on 2021-10-24},
}

@article{YOLOX,
  author    = {Zheng Ge and
               Songtao Liu and
               Feng Wang and
               Zeming Li and
               Jian Sun},
  title     = {{YOLOX:} Exceeding {YOLO} Series in 2021},
  journal   = {CoRR},
  volume    = {abs/2107.08430},
  year      = {2021},
  url       = {https://arxiv.org/abs/2107.08430},
  eprinttype = {arXiv},
  eprint    = {2107.08430},
  timestamp = {Thu, 22 Jul 2021 11:14:11 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2107-08430.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{CFPN,
  title={Smaller Object Detection for Real-Time Embedded Traffic Flow Estimation Using Fish-Eye Cameras},
  author={Ping-Yang Chen and Jun-Wei Hsieh and Munkhjargal Gochoo and Chien-Yao Wang and Hong-Yuan Mark Liao},
  journal={ICIP},
  year={2019},
  pages={2956-2960}
}

@article{YOLOv4,
  author    = {Alexey Bochkovskiy and
               Chien{-}Yao Wang and
               Hong{-}Yuan Mark Liao},
  title     = {YOLOv4: Optimal Speed and Accuracy of Object Detection},
  journal   = {CoRR},
  volume    = {abs/2004.10934},
  year      = {2020},
  url       = {https://arxiv.org/abs/2004.10934},
  eprinttype = {arXiv},
  eprint    = {2004.10934},
  timestamp = {Tue, 28 Apr 2020 16:10:02 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2004-10934.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{PP,
  author    = {Xiang Long and
               Kaipeng Deng and
               Guanzhong Wang and
               Yang Zhang and
               Qingqing Dang and
               Yuan Gao and
               Hui Shen and
               Jianguo Ren and
               Shumin Han and
               Errui Ding and
               Shilei Wen},
  title     = {{PP-YOLO:} An Effective and Efficient Implementation of Object Detector},
  journal   = {CoRR},
  volume    = {abs/2007.12099},
  year      = {2020},
  url       = {https://arxiv.org/abs/2007.12099},
  eprinttype = {arXiv},
  eprint    = {2007.12099},
  timestamp = {Wed, 29 Jul 2020 15:36:39 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2007-12099.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@software{YOLOv5,
  author       = {Glenn Jocher and
                  Alex Stoken and
                  Jirka Borovec and
                  NanoCode012 and
                  ChristopherSTAN and
                  Liu Changyu and
                  Laughing and
                  tkianai and
                  yxNONG and
                  Adam Hogan and
                  lorenzomammana and
                  AlexWang1900 and
                  Ayush Chaurasia and
                  Laurentiu Diaconu and
                  Marc and
                  wanghaoyang0106 and
                  ml5ah and
                  Doug and
                  Durgesh and
                  Francisco Ingham and
                  Frederik and
                  Guilhen and
                  Adrien Colmagro and
                  Hu Ye and
                  Jacobsolawetz and
                  Jake Poznanski and
                  Jiacong Fang and
                  Junghoon Kim and
                  Khiem Doan and
                  Lijun Yu},
  title        = {{ultralytics/yolov5: v4.0 - nn.SiLU() activations, 
                   Weights \& Biases logging, PyTorch Hub integration}},
  month        = jan,
  year         = 2021,
  publisher    = {Zenodo},
  version      = {v4.0},
  doi          = {10.5281/zenodo.4418161},
  url          = {https://doi.org/10.5281/zenodo.4418161}
}

@article{wang2022yolov7,
  title={{YOLOv7}: Trainable bag-of-freebies sets new state-of-the-art for real-time object detectors},
  author={Wang, Chien-Yao and Bochkovskiy, Alexey and Liao, Hong-Yuan Mark},
  journal={arXiv preprint arXiv:2207.02696},
  year={2022}
}
@misc{ADAM,
  doi = {10.48550/ARXIV.1412.6980},
  url = {https://arxiv.org/abs/1412.6980},
  author = {Kingma,  Diederik P. and Ba,  Jimmy},
  keywords = {Machine Learning (cs.LG),  FOS: Computer and information sciences,  FOS: Computer and information sciences},
  title = {Adam: A Method for Stochastic Optimization},
  publisher = {arXiv},
  year = {2014},
  copyright = {arXiv.org perpetual,  non-exclusive license}
}

@InProceedings{Center,
author = {Duan, Kaiwen and Bai, Song and Xie, Lingxi and Qi, Honggang and Huang, Qingming and Tian, Qi},
title = {CenterNet: Keypoint Triplets for Object Detection},
booktitle = {ICCV},
month = {October},
year = {2019}
}

@article{YOLOR,
  author    = {Chien{-}Yao Wang and
               I{-}Hau Yeh and
               Hong{-}Yuan Mark Liao},
  title     = {You Only Learn One Representation: Unified Network for Multiple Tasks},
  journal   = {CoRR},
  volume    = {abs/2105.04206},
  year      = {2021},
  url       = {https://arxiv.org/abs/2105.04206},
  eprinttype = {arXiv},
  eprint    = {2105.04206},
  timestamp = {Fri, 14 May 2021 12:13:30 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2105-04206.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@article{COCO,
  author    = {Tsung{-}Yi Lin and
               Michael Maire and
               Serge J. Belongie and
               Lubomir D. Bourdev and
               Ross B. Girshick and
               James Hays and
               Pietro Perona and
               Deva Ramanan and
               Piotr Doll{\'{a}}r and
               C. Lawrence Zitnick},
  title     = {Microsoft {COCO:} Common Objects in Context},
  journal   = {CoRR},
  volume    = {abs/1405.0312},
  year      = {2014},
  url       = {http://arxiv.org/abs/1405.0312},
  eprinttype = {arXiv},
  eprint    = {1405.0312},
  timestamp = {Mon, 13 Aug 2018 16:48:13 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/LinMBHPRDZ14.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{Focal,
  author    = {Tsung{-}Yi Lin and
               Priya Goyal and
               Ross B. Girshick and
               Kaiming He and
               Piotr Doll{\'{a}}r},
  title     = {Focal Loss for Dense Object Detection},
  journal   = {CoRR},
  volume    = {abs/1708.02002},
  year      = {2017},
  url       = {http://arxiv.org/abs/1708.02002},
  eprinttype = {arXiv},
  eprint    = {1708.02002},
  timestamp = {Mon, 13 Aug 2018 16:46:12 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1708-02002.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{SSD,
  author    = {Wei Liu and
               Dragomir Anguelov and
               Dumitru Erhan and
               Christian Szegedy and
               Scott E. Reed and
               Cheng{-}Yang Fu and
               Alexander C. Berg},
  title     = {{SSD:} Single Shot MultiBox Detector},
  journal   = {CoRR},
  volume    = {abs/1512.02325},
  year      = {2015},
  url       = {http://arxiv.org/abs/1512.02325},
  eprinttype = {arXiv},
  eprint    = {1512.02325},
  timestamp = {Wed, 12 Feb 2020 08:32:49 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/LiuAESR15.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{YOLO,
  author    = {Joseph Redmon and
               Santosh Kumar Divvala and
               Ross B. Girshick and
               Ali Farhadi},
  title     = {You Only Look Once: Unified, Real-Time Object Detection},
  journal   = {CoRR},
  volume    = {abs/1506.02640},
  year      = {2015},
  url       = {http://arxiv.org/abs/1506.02640},
  eprinttype = {arXiv},
  eprint    = {1506.02640},
  timestamp = {Mon, 13 Aug 2018 16:48:08 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/RedmonDGF15.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@misc{Pascal-Voc,
	author = "Everingham, M. and Van~Gool, L. and Williams, C. K. I. and Winn, J. and Zisserman, A.",
	title = "The {PASCAL} {V}isual {O}bject {C}lasses {C}hallenge 2012 {(VOC2012)} {R}esults",
	howpublished = "http://www.pascal-network.org/challenges/VOC/voc2012/workshop/index.html",
 }
	
@misc{darknet,
  author =   {Joseph Redmon},
  title =    {Darknet: Open Source Neural Networks in {C}},
  howpublished = {\footnotesize{\url{http://pjreddie.com/darknet/}}},
  year = {2013--2016},
}

@incollection{pytorch,
title = {PyTorch: An Imperative Style, High-Performance Deep Learning Library},
author = {Paszke, Adam and Gross, Sam and Massa, Francisco and Lerer, Adam and Bradbury, James and Chanan, Gregory and Killeen, Trevor and Lin, Zeming and Gimelshein, Natalia and Antiga, Luca and Desmaison, Alban and Kopf, Andreas and Yang, Edward and DeVito, Zachary and Raison, Martin and Tejani, Alykhan and Chilamkurthy, Sasank and Steiner, Benoit and Fang, Lu and Bai, Junjie and Chintala, Soumith},
booktitle = {Advances in Neural Information Processing Systems 32},
pages = {8024--8035},
year = {2019},
publisher = {Curran Associates, Inc.},
url = {http://papers.neurips.cc/paper/9015-pytorch-an-imperative-style-high-performance-deep-learning-library.pdf}
}

@article{paddle,
author = {Yanjun Ma and Dianhai Yu and Tian Wu and Haifeng Wang},
title = {{PaddlePaddle}: An Open-Source Deep Learning Platform from Industrial Practice},
publisher = {Frontiers of Data and Domputing},
year = {2019},
journal = {Frontiers of Data and Domputing},
volume = {1},
number = {1},
eid = {105},
numpages = {10},
pages = {105},
keywords = {;PaddlePaddle;artificial intelligence;deep learning;deep learning framework},
url = {http://www.jfdc.cnic.cn/EN/abstract/article_2.shtml},
doi = {10.11871/jfdc.issn.2096.742X.2019.01.011}
}  


